Overview of Variable Rate Coding in JPEG AI

Empirical evidence has demonstrated that learning-based image compression can outperform classical compression frameworks. This has led to the ongoing standardization of learned-based image codecs, namely Joint Photographic Experts Group (JPEG) AI. The objective of JPEG AI is to enhance compression efficiency and provide a software and hardwarefriendly solution. Based on our research, JPEG AI represents the first standardization that can facilitate the implementation of a learned image codec on a mobile device. This article presents an overview of the variable rate coding functionality in JPEG AI, which includes three variable rate adaptations: a threedimensional quality map, a fast bit rate matching algorithm, and a training strategy. The variable rate adaptations offer a continuous rate function up to 2.0 bpp, exhibiting a high level of performance, a flexible bit allocation between different color components, and a region of interest function for the specified use case. The evaluation of performance encompasses both objective and subjective results. With regard to the objective bit rate matching, the main profile with low complexity yielded a 13.1% BD-rate gain over VVC intra, while the high profile with high complexity achieved a 19.2% BD-rate gain over VVC intra. The BD-rate result is calculated as the mean of the seven perceptual metrics defined in the JPEG AI common test conditions. With respect to subjective results, the example of improving the quality of the region of interest is illustrated.

==> sections/delete_temp.tex <==
\label{sec:Channel-wise}
\begin{figure}
    \centering
    \includegraphics[width=0.48\textwidth]{picture/BDL.pdf}
    \caption{The illustration demonstrates the use of four models to generate an optimal variable rate curve and the use of a single model to cover a large bit rate range. }
    \label{fig:BDL}
\end{figure}

In JPEG-AI, to cover a large bit rate range, there are four models trained for a specific Lagrange multiplier $\beta_\mathrm{train}$ determining rate-distortion trade-off as described in (\ref{eq_2}). A higher value of $\beta_\mathrm{train}$ yields a higher quality reconstructed image, requiring more bits to code. 
The rationale behind utilising four models is explained in Fig. \ref{fig:BDL}, which depicts three distinct lines. The orange line illustrates the process of employing four models to construct an optimal variable rate envelope. The curve represents four points, each denoting a model that has been trained with a distinct $\beta_\mathrm{train}$ and encoding with the $\beta_\mathrm{test} = \beta_\mathrm{train}$. These points are referred to as anchor points.

In Fig. \ref{fig:BDL}, the blue and green curves illustrate the generation of multiple bit rate points using a single model. The two curves were generated using the same model, which is the third model from the left on the orange curve. The blue curve illustrates the performance of the relatively lower bit rate range, while the green curve depicts the performance of the relatively higher bit rate range. From this figure, we can observe the following characteristics:    
\begin{description}
  \item[$\bullet$]Firstly, it is feasible to utilise a single model to encompass a broad bit rate range.
  \item[$\bullet$]Secondly, the single model exhibits optimal performance when the bit rate range is proximate to the anchor point.
  \item[$\bullet$]Thirdly, if the single model provides a bit rate that is either too low or too high in comparison to the anchor point, the resulting performance will not meet the desired specifications.
  \item[$\bullet$]Fourthly, when providing a higher bit rate than the anchor point from the single model, the performance decline is more rapid than when providing a lower bit rate.
  \item[$\bullet$]Finally, the method of providing a variable rate for a single model is based on the alteration of quantization steps. In the region of the higher bit rate, the BD-rate performance is already saturated when the rate is increased. This phenomenon can be explained by the fact that autoencoders are lossy systems even in the absence of quantization. Increasing the quantization step size will not result in improved model performance after a certain point.
\end{description}

In consideration of the aforementioned listing features, we proposed that four models be utilized in order to provide coverage across a broad bit rate range, thereby enhancing the variable rate performance. In order to facilitate the implementation of the variable rate function in a hardware-friendly manner, we undertook the following adaptations, taking into account the variable rate feature. 


% variable rate feature
By observing the variable rate feature in Fig. ??, in order to enable a single model to provide a variable rate with optimal performance, the value of the parameter $\Delta_{\beta}$ is constrained to lie within the interval $[−1069, 702]$. The lower and upper bounds of this interval are determined based on empirical observations. By imposing a limit on the value of $\Delta_{\beta}$ , each model is constrained to a specific range of bit rates, necessitating the use of four models to encompass the entire range of bit rates. When the codec is required to achieve a specified target rate, a strategic approach is necessary to select an appropriate model and provide the corresponding $\Delta_{\beta}$ value. The following subsection will introduce the bit rate matching algorithm.

==> sections/introduction.tex <==
\section{Introduction}
\IEEEPARstart{t}{he} consumption of online media is increasing, leading to a growing need for high-quality content with lower bitrates~\cite{ma2019image,birman2020overview}. The increasing need for media has resulted in the swift advancement of traditional and neural network-based image codecs. In terms of rate distortion performance, the early NN-based codecs~\cite{balle2017end,balle2018variational,minnen2018joint,liu2019non,zhou2019multi,cui2021asymmetric,lee2018context,mentzer2018conditional,cheng2020learned,qian2020learning,9067005,koyuncu2021parallel,he2021checkerboard,minnen2020channel,qian2021entroformer} are comparable to traditional standards such as JPEG~\cite{wallace1992jpeg}, JPEG2000~\cite{skodras2001jpeg} and BPG~\cite{bellard2015bpg} (an intra coding of HEVC~\cite{sze2014high}). Furthermore, the recently proposed NN-based image codecs~\cite{he2022elic,guo2021causal,koyuncu2022contextformer} have already surpassed the intra coding of state-of-the-art video coding standards, such as VVC~\cite{ohm2018versatile}. 

The NN-based image codecs, such as~\cite{balle2017end,balle2018variational,minnen2018joint,liu2019non,zhou2019multi,cui2021asymmetric,lee2018context,mentzer2018conditional,cheng2020learned,qian2020learning,9067005,koyuncu2021parallel,he2021checkerboard,minnen2020channel,qian2021entroformer,guo2021causal,he2022elic,koyuncu2022contextformer,liu2023learned}, utilize an autoencoder framework. An autoencoder framework contains a non-linear transformation~\cite{balle2020nonlinear}. The autoencoder framework features a forward-backward adaptive entropy model~\cite{balle2018variational} that generates a latent representation of an image with low entropy. 
The adaptation process in the entropy model is based on a signaled prior. The contextual information extracted by an autoregressive context model~\cite{minnen2018joint} is used for the backward adaptation of the entropy model. 



The conditional autoencoder framework is a widely used method for compressing images and videos with great success. A conditional autoencoder can use auxiliary information to enhance the reconstructed quality. To exemplify, Li et al. put forth the concept of DCVC~\cite{li2021deepcontextualvideocompression}, which employs conditional coding in the inter-prediction of video codecs. Moreover, Ladune et al. proposed a new inter-frame coding technique~\cite{Ladune2020OpticalFA} that utilizes two complementary autoencoders, called \textit{MOFNet} and \textit{CodecNet}. MOFNet predicts the subsequent frame by utilizing optical flow. CodecNet is a conditional autoencoder that effectively captures the dependencies between the original and predicted frames by utilizing MOFNet's prediction as auxiliary information. Brand et al. use a conditional encoder for image compression in their work~\cite{9244548} on image compression. The conditional encoder utilizes pixels from the local neighbourhood as auxiliary information, given the absence of motion prediction in this scenario. The image input is divided into $16 \times 16$ blocks, and the encoder is conditioned using an area that is four pixels wide around each block. We proposed a so called conditional colour separation (CCS) framework in~\cite{jia2022learningbased}, that can parallel process the different colour components based on conditional autoencoder structure. In the CCS framework, different colour components are separated into the primary and secondary group. Two different colour components will be processed in parallel, additionally, the secondary colour components processing requires the auxiliary information that comes from the primary colour components. The CCS framework allows parallel processing for the different colour components, and can assign different complexity to each colour components codec by varying the number of channels for each group of components. \IEEEpubidadjcol

The aforementioned image compression codecs,~\cite{balle2017end,balle2018variational,minnen2018joint,liu2019non,zhou2019multi,cui2021asymmetric,lee2018context,mentzer2018conditional,cheng2020learned,qian2020learning,9067005,koyuncu2021parallel,he2021checkerboard,minnen2020channel,qian2021entroformer,guo2021causal,he2022elic,koyuncu2022contextformer,liu2023learned,jia2022learningbased}, are limited in their ability to provide continuous rate control through the utilisation of a single model. Instead, they are only capable of obtaining multiple models for varying quality levels through the incorporation of distinct quality parameters within the loss function during training. In order to facilitate the implementation of continuous variable rate functionality for the learned image codec, a number of approaches have been put forth for consideration~\cite{choi2019variable,song2021variable,9522770,Cui2020GVAEAC,cui2021asymmetric}. For instance, Choi et al.~\cite{choi2019variable} and Song et al.~\cite{song2021variable} introduce conditional transform layers, where the transforms are adaptively modified according to the target rate. Moreover, the model of~\cite{song2021variable} can allocate more bits for the region of interest to increase coding quality on a selected location. Brand et al.~\cite{9522770} proposed a pyramidal NN structure with latent masking. Finetuning the mask for each layer allows for variable rate coding. Alternatively, the model of~\cite{Cui2020GVAEAC,cui2021asymmetric} proposes a so called \textit{gain unit}, which directly adjusts the latent variables without requiring modifications to the transform layers.

The CCS framework is employed as the foundational framework within the JPEG AI standardisation verification model (VM). Moreover, the gain unit based channel-wise quality map and an additional spatial quality map ~\cite{jia2024bitdistributionstudyimplementation} are employed in JPEG AI to facilitate the variable rate functionality. In order to evaluate the BD-rate performance, seven quality metrics are employed, including MS-SSIM~\cite{1292216}, Visual Information Fidelity (VIF)~\cite{citVif}, feature similarity (FSIM)~\cite{5705575}, Normalized Laplacian Pyramid (NLPD)~\cite{nlpdcite}, Information Content Weighted Structural Similarity Measure (IW-SSIM)~\cite{5635337}, Video Multimethod Assessment Fusion (VMAF)~\cite{VMAFcite}, and PSNR-HVS-M~\cite{psnrHVS}. 

The implementation of an adaptive training strategy and bit rate matching algorithm has enabled the base operation point of JPEG AI to achieve, on average across seven metrics, a 13.1\% BD-rate gain over the VVC intra mode. Furthermore, the high operation point with high complexity has demonstrated the capacity to achieve a 19.2\% BD-rate gain over VVC intra on average across seven metrics. Moreover, the spatial quality map can enhance the subjective quality of the region of interest.


The following section presents an overview of related works in the field of learned image codecs and variable rate functions. Section \RomanNumeralCaps{3} outlines the variable rate adaptions in JPEG AI. Section \RomanNumeralCaps{4} describes the experiments and the experimental results, while Section \RomanNumeralCaps{5} presents the conclusions.

The following functions of JPEG AI are the focus of this article: 

\begin{description}
  \item[$\bullet$] A 3D quality map of the identical size to that of the latent tensor can be generated through the extension of a channel-wise quality map, a spatial quality map, or a combination of both.
  \item[$\bullet$] The channel-wise quality map is employed to facilitate an overall rate control, thereby enabling the model to achieve a continuous variable rate. By collaborating with a efficient bit rate alignment algorithm, the model is capable of precisely matching to a targeted rate point with optimal performance. 
  \item[$\bullet$] A spatial quality map is employed as a means of facilitating flexible spatial bit allocation. In order to reduce the number of signal bits, a series of entropy simplifications of the spatial quality map is introduced. 
  \item[$\bullet$] A training strategy comprising distinct stages was introduced, with each stage encompassing a unique training parameter. This approach was designed with the objective of enhancing overall performance and facilitating variable rate adaptation.
\end{description}





%%%%%old jpeg history
The favorable performance of the learned-based codecs has generated considerable interest from both industrial and academic circles. This has resulted in the ongoing standardization of JPEG AI \cite{ascenso2021white}. The scope of the JPEG AI is the creation of a learning-based image coding standard offering a single-stream, compact compressed domain representation, targeting both human visualization, with significant compression efficiency improvement over image coding standards in common use at equivalent subjective quality, and effective performance for image processing and computer vision tasks, with the goal of supporting a royalty-free baseline. 
In 2019, the JPEG Standardization Committee initiated JPEG AI to define the first image coding specifications, taking advantage of an end-to-end learning-based coding approach. The JPEG AI specifications will be soon published as an International Standard in early 2025. JPEG AI exploits the current state-of-the-art in deep learning while taking into account considerations for a deployment in a near-future. Therefore, JPEG AI design was refined in several iterations to reach the level of maturity and feasibility to both encode and decode images on mobile devices. 
